Caption Feature Space Regularization for Audio Captioning

Audio captioning aims at describing the content of audio clips with human language. Due to the ambiguity of audio, different people may perceive the same audio differently, resulting in caption disparities (i.e., one audio may correlate to several captions with diverse semantics). For that, general audio captioning models achieve the one-to-many training by randomly selecting a correlated caption as the ground truth for each audio. However, it leads to a significant variation in the optimization directions and weakens the model stability. To eliminate this negative effect, in this paper, we propose a two-stage framework for audio captioning: (i) in the first stage, via the contrastive learning, we construct a proxy feature space to reduce the distances between captions correlated to the same audio, and (ii) in the second stage, the proxy feature space is utilized as additional supervision to encourage the model to be optimized in the direction that benefits all the correlated captions. We conducted extensive experiments on two datasets using four commonly used encoder and decoder architectures. Experimental results demonstrate the effectiveness of the proposed method. The code is available at https://github.com/PRIS-CV/Caption-Feature-Space-Regularization.

==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Abstract.tex <==
\begin{abstract}
% The goal of the audio captioning task is to create a description of the audio clips' contents. Due to the ambiguity of audio, multiple people may perceive the same audio differently, resulting in caption disparities. However, because the audio captioning task uses a one-to-many training strategy, the disparity in captions has an impact on description generation, causing the network to become unstable. So in order to solve this problem, we propose a two-stage caption semantic consistency constraint method for audio captioning. Stage 1 use contrast learning to construct the caption semantic space and extract the caption semantic embedding, while stage 2 employs the  semantic embedding to regularize caption generation and reduce the effects of training approach and disparity. We conducted extensive experiments on two datasets using four commonly used encoder and decoder models. Experimental results indicate that the effectiveness of our proposed method in the metrics.

Audio captioning aims at describing the content of audio clips with human language. Due to the ambiguity of audio, multiple people may perceive the same audio differently, resulting in caption disparities (\emph{i.e.}, one audio may correlate to several captions with diverse semantics). For that, general audio captioning models achieve the one-to-many training by randomly selecting a correlated caption as the ground truth for each audio. However, it leads to a significant variation in the optimization directions and weakens model stability. To eliminate this negative impact, in this paper,  we propose a two-stage framework for audio captioning: (i) in the first stage, via a caption consistency regularization, we construct a proxy feature space to reduce distances between captions correlate to the same audio, and (ii) in the second stage, the proxy feature space is used as additional supervision to encourage the model to be optimized in a direction that benefits all correlated captions. We conducted extensive experiments on two datasets using four commonly used encoder and decoder architectures. Experimental results indicate the effectiveness of our proposed method in the metrics.
\end{abstract}

\begin{IEEEkeywords}
Audio captioning, contrastive learning, cross-modal task, semantic consistency constraint
\end{IEEEkeywords}


==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Conclusion.tex <==
\vspace{-10pt}
\section{Conclusion}
In this paper, we propose a two-stage caption semantic consistency constraint method for the audio captioning task, in which stage 1 uses contrast learning to extract the common semantic embedding of audio captions and stage 2 uses the extracted semantic embedding to regular the generated of caption and mitigate the impact of the caption disparity. We perform experiments using four different combinations of pre-trained encoders and decoders on two datasets to demonstrate the performance and effectiveness of our approach. According to the results, our best model performs competitive performance to the SOTA method on the Clotho-v1 dataset and outperforms the SOTA method on the Clotho-v2 dataset.

==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Experiments.tex <==
\vspace{-15pt}
\section{Experiments}
\vspace{-10pt}
\subsection{Metrics}
We evaluate the performance of our proposed method using the same metrics adopted in the DCASE Challenge, including machine translation metrics: BLEU$_n$~\cite{papineni2002bleu}, METEOR~\cite{banerjee2005meteor}, ROUGE$_L$~\cite{lin2004rouge} and captioning metrics: CIDEr~\cite{vedantam2015cider}, SPICE~\cite{anderson2016spice}, SPIDEr~\cite{liu2017improved}. 

The machine translation metrics are used to measure the word accuracy and recall of generated text compared to the ground truth, $n$ in BLEU means $n-$gram. And the captioning metrics are designed for the captioning task, which takes into account the scene graph inside the generated caption and the term frequency-inverse document frequency (TF-IDF) of the n-gram. By considering the scene graph and the TF-IDF of n-gram, ensuring semantic fidelity and syntactic fluency of the generated captions.
\vspace{-10pt}
\subsection{Datasets}

The Clotho dataset~\cite{drossos2020clotho} and the Audiocaps dataset~\cite{kim2019audiocaps} are two datasets that are commonly used for audio captioning tasks. There are two versions of the Clotho dataset, Clotho-v1 and Clotho-v2 respectively. each audio clip has five captions describing the audio contents, and the annotator uses only the audio signal for annotation. However, the Audiocaps dataset is not generated in an ideal environment, where annotators are provided with word labels and video information in addition to the audio signal~\cite{kim2019audiocaps}. So in this work,we only focus on the Clotho-v1 and Clotho-v2 datasets.
\vspace{-10pt}
\subsection{Experimental results}
Table I illustrates the experimental results of the proposed method compared to the baseline model and other methods on the Clotho-v1 and Clotho-v2 evaluation sets.

In each table, the first major column shows the experimental results of baseline models with different combinations of encoders and decoders, and the second major column is the result of other state of the art methods, where the baseline model using Pretrain-CNN encoder and attention-based GRU decoder is our implementation of the AT-CNN method. And the last major column is the experimental results of our proposed semantic consistency constraint method.

\subsubsection{Compared with baseline models}In both two datasets, our proposed semantic consistency constraint methods outperform the baseline models in the same encoder and decoder models. When compared to the SOTA model, AT-CNN, our best model which the encoder is Pretrain-CNN and the decoder is GRU, performs similarly on the Clotho-v1 dataset and outperforms it on the Clotho-v2 dataset.

\subsubsection{Compared with other methods}From the results, our proposed model has a generally higher performance improvement on the Clotho-v2 dataset compared to Clotho-v1 in terms of captioning metrics. We believe this is because the Clotho-v2 dataset is larger than the Clotho-v1 dataset, which aids in the extraction of caption semantic embedding in stage 1 and hence minimizes the impact of caption disparity on caption creation and enabling the generated captions to achieve better performance in captioning metrics.




==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Introduction.tex <==
\vspace{-15pt}
\section{Introduction}

\IEEEPARstart{a}{udio}  captioning is an inter-modal translation task that requires extracting features from audio and combining them with a language model to describe the contents of audio~\cite{drossos2017automated,drossos2020clotho,koizumi2020transformer}. However, unlike the speech recognition task that transcribes speech to text~\cite{xu2021audio}, the audio captioning task focuses on recognizing human-perceived information in general audio signals and expressing it in text using natural language. The information includes the sound event, the acoustic scene, and high-level semantic information such as concepts, physical properties, and high-level knowledge~\cite{drossos2020clotho}.

% The audio captioning task is first introduced in~\cite{drossos2017automated}, which proposed the commercial ProSound Effects~\cite{lipping2019crowdsourcing} audio corpus as a proof of concept. The paper proposed a BiGRU~\cite{rana2016gated} based encoder-decoder model to generate audio captions. And due to the success of the audio captioning task in DCASE 2020 and 2021~\cite{Drossos_2019_dcase}, this task has garnered the attention of an increasing number of researchers, several papers and methods to address this issue have been proposed. H. Wang et al.~\cite{helinautomated} proposed a temporal attention mechanism in the decoder, which could utilize more acoustic information for each time step. K. Chen et al.~\cite{chen2020audio} used the combination of a pre-trained encoder and a Transformer decoder which makes the latent variable resulted more efficient in generating captions. X. Xu et al.~\cite{xu2021investigating} investigated the impact of local and global information on the audio captioning task by comparing two pre-training tasks. The semantic information is also studied to improve the performance of the audio captioning task. the semantic attributes are firstly used in ~\cite{kim2019audiocaps}, which used AudioSet labels as semantic attributes by using the labels of the nearest video clip. And  Eren et al. ~\cite{eren2020audio} used the audio encoder to get audio embeddings and text encoder to get subject-verb embeddings, combine these embeddings and decode them in the decoder.

Different from the visual captioning tasks in which people can easily describe the visual object by its shape, color, size, and its position relative to other objects~\cite{wu2019audio}. However, for the audio sounds, its information can be much more ambiguous than the information in the image or video~\cite{drossos2020clotho,wu2019audio}. Even people find it challenging to precisely detect the events in an audio signal. Furthermore, it is difficult to determine the ideal description for the given audio because the description is often dependent on the situation or context as much as the sound itself. But due to the ambiguity of audio, different persons may have varying perceptions of the same sounds, resulting in the semantic disparity of audio captions~\cite{drossos2020clotho}, for example, a thin plastic rattling could be perceived as a fire crackling~\cite{lipping2019crowdsourcing}.

In the audio captioning task, each audio has multiple captions to describe the contents, and one caption for each training is randomly selected as the objective for the model to generate a description of the audio clip. However, due to the disparity of captions, randomly selecting one caption as the objective during each training will lead to a large variance in the optimization direction of the model, which may have a significant impact on the performance of the model and make it more difficult to train.
% \textcolor{blue}{However due to the disparity of captions, this one-to-many training strategy may have a significant impact on the performance of the model and make it more difficult to train. }

To solve the problem caused by the disparity of captions, the most intuitive way is to feed all captions of each audio simultaneously as optimization objectives into the network at the same time for training, but this approach leads to a multiply increasing memory, which is not an acceptable solution with limited computational resources.

\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_2.png}}
\caption{The system overview of our proposed method. The mainstream encoder-decoder audio captioning framework is in the yellow block, and in the green block is our proposed  caption semantic consistency constraint module which is described in sections B and C.}
\vspace{-13pt}
\end{figure*}
So we choose not to impose this stability constraint at the model output level, but to reconstruct such a constraint in the feature space. We propose a two-stage caption semantic consistency constraint method. Our proposed method includes two-stage: stage 1 generates the semantic space of the captions by minimizing the distance between different captions belonging to the same audio and pushing away the distance between different captions of different audio. And stage 2 regularizes the creation of audio descriptions by using the semantic feature space generated in stage 1 as our optimization objective.

% the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and extract the common caption semantic embedding of each audio. And in order to mitigate the influence of the training strategy, stage 2 regularizes the generation of audio captions using the extracted caption semantic embedding.


Our contributions are as follows:
\begin{itemize}
  \item [1)] We propose a two-stage caption semantic consistency constraint approach to mitigate the impact of caption disparity on audio captioning tasks.
  \item [2)]Two different pre-trained encoders and two different decoders are used to verify the effectiveness of the method.
  \item [3)]On two prominent audio captioning datasets, Clotho-v1 and Clotho-v2~\cite{drossos2020clotho}, the results of our proposed method are compared to the results of the state of the arts, indicating that our proposed method achieves competitive results.
\end{itemize}

% The remainder of this paper is organized as follows. We introduce our proposed method in Section 2. Experiments are described in Section 3. Results are shown in Section 4. Finally, we conclude our work in Section 5.


==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Method.tex <==
% \begin{figure*}
% \centerline{\includegraphics[width=14cm]{stage_1.pdf}}
% \caption{The system overview of stage 1. Different colors indicate caption embeddings from different audios.}
% \end{figure*}
\section{Proposed Method}
The proposed model, which is a two-stage method, is described in this section. Stage 1 uses contrast learning to extract the common semantic embedding of audio captions, reducing the impact of caption semantic disparity. Stage 2 constrains the generated audio description using the extracted semantic embedding.
\subsection{Stage 1:The extraction of caption semantic embedding}
To reduce the impact of caption disparity on model training due to training strategy. We use the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and increase the semantic space distance between captions that belong to different audio.
\subsubsection{Training method}
As is depicted in Fig. 1, $N \times M$ captions are fetched to build a batch. These captions are from $N$ different audios, and each audio has $M$ captions. The symbol $t_{ji}$ ($1 \le j \le N$ and $1 \le i \le M$) represents the $i$th caption from the $j$th audio. 

We tokenize the captions and utilize Bert~\cite{devlin2018bert} to extract the its word embeddings. And then the word embeddings are fed into an LSTM network. A linear layer is connected to the LSTM layer as an additional transformation of the network. We denote the output of the entire neural network as $ G\left ( t_{ji};w \right ) $ where $w$ represents all parameters of the neural network. The caption embedding vector is defined as:
\begin{equation}
e_{ji} = Mean\left ( G\left ( t_{ji};w \right ) \right ) + Max\left ( G\left ( t_{ji};w \right ) \right ),
\end{equation}
here $e_{ji}$ represents semantic embedding of the $j$th audio’s $i$th caption. 

The centroid of the semantic embeddings from the $j$th audio $\left [ e_{j1},\cdots ,e_{jM} \right ] $ is denoted as $c_{j}$, and the similarity matrix $S_{ji,k}$ is defined as the scaled cosine similarities between each semantic embedding $e_{ji}$ to all centroids $c_{k}$ ($1 \le j, k \le N$ and $1 \le i \le M$):
\begin{equation}
S_{ji,k}= w \cdot cosine\left ( e_{ji},c_{k} \right ) +b ,
\end{equation}
where $w$ and $b$ are learnable parameters, the weight are constrained to be positive ($w > 0$). And the centroid $c_{k}$ can be calculated by:
\begin{equation}
c_{k} = \left\{\begin{array}{ll}
\frac{1}{M} \cdot \sum_{m=1}^{M}e_{k m},&if \ k \neq j  \\
\frac{1}{M-1} \cdot \sum_{m=1,m \neq i}^{M}e_{k m}, & if \ k =j
\end{array}\right.
\end{equation}
In Eqn.3, when calculating negative similarity ($k \neq j$), the centroid $c_{k}$ is the average of all the
semantic embeddings of $k$th audio, while when calculating positive similarity ($k = j$), we eliminate $e_{ki}$ to compute the centroid.

During the training, we want the semantic embeddings of each audio to be similar to its centroid, but far from the centroid of other audios in the semantic space. As shown in the similarity matrix in Fig. 1, we want the similarity values of colored areas to be large, and the values of blank areas to be small. So for each semantic embedding, the loss function is designed as:
\begin{equation}
L\left(\mathbf{e}_{j i}\right)=-\mathbf{S}_{j i, j}+\log \sum_{k=1}^{N} \exp \left(\mathbf{S}_{j i, k}\right).
\end{equation}

After the training of stage 1 is completed, we extract the centroid of each audio to represent its caption semantic embedding.
\subsubsection{Training details}
In this stage, we use a single-layer, bi-directional LSTM network followed by a linear fully connected layer, The dimensions of the LSTM and linear layer are 1024 and 512, respectively. When training the  model, each batch contains $N$ = 64 audios and $M$ = 3 caption per audios. We train the network with Adam optimizer using a learning rate of 0.01, and the total number of training epochs is 500. The scaling factors ($w$,$b$) are initialized as ($10$,$-5$).
\subsection{Stage 2:The generation of audio captioning}
%总述目前的模型一般Seq2Seq的
Existing audio captioning systems are usually based on an encoder-decoder framework, as shown in Fig. 2. In the encoder, the audio data is encysted into a latent representation, and then the representation is fed to the decoder for word-level prediction to generate captions for audio.
\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_2.pdf}}
\caption{The system overview of stage 2. }
\end{figure*}

Typically, the encoder employs pre-trained models that have been trained in advance for sound event detection or sound scene recognition tasks, such as PANN~\cite{kong2020panns}, VGGish~\cite{hershey2017cnn}, or Pretrain-CNN~\cite{xu2021investigating}. And the decoder is an autoregressive language model, like Transformer or GRU, which is trained from scratch.
\subsubsection{Encoder}
In our work, we used two different 10-layer CNN pre-training models, PANN and Pretrain-CNN, and the model structures are shown in Table I.
% \begin{table}[h]
%     \caption{Caption}
%     \label{tab:my_label}
%     \centering
%     \begin{tabular}{c|c}\hline
%     PANN & Pretrain-CNN\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                         3 \times 3 @ 64 \\ BN, ReLU 
%                         \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                     3 \times 3 @ 128 \\ BN, ReLU 
%                     \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                 3 \times 3 @ 256 \\ BN, ReLU 
%                 \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%             3 \times 3 @ 512 \\ BN, ReLU 
%             \end{array}\right) \times 2$}\\\hline
%     Global pooling & Pooling with length  \\\hline
%     \multicolumn{2}{c}{FC 512,ReLU}\\\hline
%     \multicolumn{2}{c}{FC 527, Sigmoid}\\\hline
    
%     \end{tabular}

% \end{table}

Both PANN~\cite{kong2020panns} and Pretrain-CNN~\cite{xu2021investigating} are pre-trained on Audioset, the world's biggest sound event detection dataset. The distinction is that Pretrain-CNN computes the representation using the actual length of each audio feature, whereas PANN during training uses the longest length in the batch.

\subsubsection{Decoder}We use a single-layer attention-based  GRU~\cite{bahdanau2014neural} and 2 layers transformer~\cite{vaswani2017attention} as our backbone decoder for its success in previous audio captioning works.

% \emph{GRU Decoder:} At the each decoding step $n$, the hidden state $h_{n}$ is updated depending on the previous timestep $h_{n-1}$, and the concatenation of the current input word token $t_{n}$ and a context vector $v_{n}$:
% \begin{equation}
% h_{n}=GRU\left(\left[v_{n} ;WE\left(t_{n}\right)\right], h_{n-1}\right),
% \end{equation}
% where $WE$ denotes the word embedding layer. A standard temporal attention mechanism is utilized to obtain $v_n$ the attention weights $\left \{\alpha_{n,t} \right \} ^{T}_{t=1}$ can be calculated by $h_{n-1}$ and the audio representation:
% \begin{equation}
%     \alpha_{n, t}=\frac{\exp \left(score\left(\mathbf{h}_{n-1}, \mathbf{e}_{t}\right)\right)}{\sum_{t=1}^{T^{\star}} \exp \left(score\left(\mathbf{h}_{n-1}, \mathbf{e}_{t}\right)\right)},
% \end{equation}
% \begin{equation}
%     v_{n}= {\sum_{t=1}^{T}\alpha_{n, t}\cdot e_{t}}.
% \end{equation}

% \emph{Transformer Decoder:} In our work, we use the typical 2 layers  Transformer decoder, The detailed
% structure of Transformer can be found \textcolor{blue}{in}.

% \textcolor{blue}{The word embedding of the token is fed into the decoder. The input is delivered to the masked multi-head attention module, which generates a query vector feature using a decoder layer. The value vector is then used as an input to the subsequent multi-head attention module. Additionally, the multi-head attention module uses encoder output as the key vector and value vector inputs. We may retrieve the output of a decoder layer after layer norm and feedforward module. Each decoder layer employs a skip connection method to avoid gradient vanishing difficulties. Finally, the decoder's output is transferred to a linear layer and a softmax function to obtain the caption words' output probabilities.}
\subsubsection{Loss}
We use the combination of two loss functions in the training, the standard cross-entropy loss  and the semantic constraint loss.

\emph{Cross-entropy Loss:} The cross-entropy loss function is used for word-level classification, for the same reason as other audio captioning methods use. Given the acoustic feature $F$ of the audio, the parameters of the model are $w$, the loss function is:
\begin{equation}
    \ell_{\mathrm{CE}}(\omega  ; S, F)=-\sum_{t=1}^{T} \log p\left(S_{t} \mid \omega , F\right),
\end{equation}
where $S$ is the objective caption of the audio and $S_{t}$ is the expected word at time $t$.

\emph{Semantic Constraint Loss:} We obtain the semantic embedding of the generated caption by averaging pooling and max pooling operations on the decoder output feature $H$ along the time axis, as shown in the following equation:
% In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity. 
% We obtain the semantic embedding of the generated caption by averaging pooling and max pooling operations on the decoder output feature $H$ along the time axis, as shown in the following equation:
\begin{equation}
    \hat{e}_{k}(\omega,F) = Mean\left (H(\omega,F) \right ) + Max\left ( H(\omega,F) \right ),
\end{equation}
where $\hat{e}_{k}$ is the semantic embedding of the $k$th audio generated caption.

In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity (see Equation 10). 
\begin{equation}
    \ell_{SC}(\omega  ; c_{k}, F) = 1 - cosine\_similarity(\hat{e}_{k},c_{k}),
\end{equation}
 In this way, a small loss means $\hat{e}_{k}$ has high similarity with the audio caption semantic embedding $c_{k}$ obtained by stage 1.
 
Accordingly, the final training objective function is the weighted sum of cross-entropy loss and semantic constraint loss, where $\lambda$ is a hyperparameter.
\begin{equation}
 \ell(\omega; c_{k}, S, F) = \ell_{\mathrm{CE}}(\omega  ; S, F) + \lambda \cdot \ell_{SC}(\omega  ; c_{k}, F)
\end{equation}

\subsubsection{Training details} \textcolor{blue}{In this stage, we apply SpecAugment~\cite{park2019specaugment} before feeding the audio feature to the model. Label smoothing~\cite{szegedy2016rethinking} is applied to smooth the one-hot word label. We also apply scheduled sampling to gently decrease the training-inference discrepancy caused by teacher forcing training~\cite{bengio2015scheduled}. The probability of feeding the ground truth word to the decoder is linearly decayed from 1.0 to 0.7. We train the network with Adam optimizer using initial learning rate $5e^{-5}$, and the total number of training epochs is 25. }


==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/NewMethod.tex <==
\vspace{-15pt}
\section{Proposed Method}

\subsection{The overview of audio captioning system}
the current mainstream training paradigm of the audio captioning task is the end-to-end encoder-decoder framework, as shown in the yellow block of Fig. 1.

The training data for the task consists of paired audio and captions data. We denote a training set of $N$ audio-captions pair $D=\left\{\left(x_{n}, C_{n}\right)\right\}_{n=1}^{N}$, where $x\in {R}^{T \times F}$ is the log mel-spectrogram of the audio clip with $T$ frames and $F$ Mel filters, $C_n=\left\{c_{mn}^{L}\right\}_{m=1}^{M}$ is all the captions of the $n$th audio clip, and $c_{mn}^{L}$ is the $m$-th caption having $L$ tokens.

The audio encoder takes the log mel-spectrogram $x$ of an audio clip as the input and extracts its latent representation $z\in {R}^{T^{\prime} \times F^{\prime}}$. Then latent representation $z$ is aligned and calculated with the hidden states of tokens by the decoder, the caption representation can be calculated by the decoder, denoted as $H \in {R}^{L \times D}$, which contains $L$ vectors $\left\{h_l\right\}_{l=1}^{L}$, where the dimension of $h_l$ is $D$ and the  number of vectors is equal to the token length of caption $c$. Hence, each vector $h_l$ corresponds to the token $c^l$ in the objective caption, and then the vectors are  used to predict the probability of the words over the vocabulary after it is passed through the  linear layer with softmax function.The predicted words are $\left\{w_l\right\}_{l=1}^{L}$.

The cross-entropy loss function is used for word-level classification of decoder, the loss function is:
\begin{equation}
    \ell_{\mathrm{CE}}(\theta  ; c, x)=-\sum_{l=1}^{L} c^l \cdot \log p\left(w_{l} \mid \theta, x\right),
\end{equation}


\subsubsection{Encoder}
The encoder employs pre-trained models that have been trained in advance for sound event detection or sound scene recognition tasks, such as PANN~\cite{kong2020panns}, VGGish~\cite{hershey2017cnn}, or Pretrain-CNN~\cite{xu2021investigating}. And in our work, we used two different 10-layer CNN pre-trained models, PANN and Pretrain-CNN, and the model structures of them can be found in ~\cite{kong2020panns,xu2021investigating}.

\subsubsection{Decoder}The decoder is usually a language model, like Transformer or GRU, which is trained from scratch. And during training, teacher forcing is used to accelerate the training process. In our work, we use a single-layer attention-based  GRU~\cite{bahdanau2014neural} and 2 layers transformer~\cite{vaswani2017attention} as our backbone decoder for its success in previous audio captioning works.

For the audio captioning task, an audio clip has multiple captions to describe how different annotators feel about it. Different perceptions cause the disparity of the captions, however, for each audio, only one caption will be randomly selected as the groundtruth for each training to generate the description of the audio, and this training strategy can easily affect the performance of the model and make it unstable.

To solve the above problem, we propose a caption semantic consistency constraint method to regularize the generation of the caption, the key module are shown in the green block of Figure 1. Our method is a two-stage audio captioning method, in which stage 1 uses contrast learning to generate the semantic space and extract the caption semantic embedding of each audio $d_k$ (described in section B) and then the semantic embedding $d_k$ is used in the module to regularize the generation of caption in stage 2 (described in section C).
\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_1.png}}
\caption{The system overview of stage 1. Different colors indicate caption embeddings from different audios. The colored areas are the positive similarity and the blank areas are negative in the similarity matrix.}
\vspace{-13pt}
\end{figure*}\textbf{}


\vspace{-10pt}
\subsection{Stage 1:The extraction of caption semantic embedding}
To reduce the impact of caption disparity on model training. We use the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and increase the semantic space distance between captions that belong to different audio.

\subsubsection{Training method}
As is depicted in Fig. 2, $N \times M$ captions are fetched to build a batch. These captions are from $N$ different audios, and each audio has $M$ captions. The symbol $c_{ji}$ ($1 \le j \le N$ and $1 \le i \le M$) represents the $i$th caption from the $j$th audio. 

We tokenize the captions and utilize Bert~\cite{devlin2018bert} to extract its word embeddings. And then the word embeddings are fed into an LSTM network. A linear layer is connected to the LSTM layer as an additional transformation of the network. We denote the output of the entire neural network as $ G\left ( c_{ji};w \right ) $ where $w$ represents all parameters of the neural network. The caption embedding vector is defined as:
\begin{equation}
e_{ji} = Mean\left ( G\left ( c_{ji};w \right ) \right ) + Max\left ( G\left ( c_{ji};w \right ) \right ),
\end{equation}
here $e_{ji}$ represents semantic embedding of the $j$th audio’s $i$th caption. 

The centroid of the semantic embeddings from the $j$th audio $\left [ e_{j1},\cdots ,e_{jM} \right ] $ is denoted as $d_{j}$, and the similarity matrix $S_{ji,k}$ is defined as the scaled cosine similarities between each semantic embedding $e_{ji}$ to all centroids $d_{k}$ ($1 \le j, k \le N$ and $1 \le i \le M$):
\begin{equation}
S_{ji,k}= w \cdot cosine\left ( e_{ji},d_{k} \right ) +b ,
\end{equation}
where $w$ and $b$ are learnable parameters, the weight are constrained to be positive ($w > 0$). And the centroid $c_{k}$ can be calculated by:
\begin{equation}
d_{k} = \left\{\begin{array}{ll}
\frac{1}{M} \cdot \sum_{m=1}^{M}e_{k m},&if \ k \neq j  \\
\frac{1}{M-1} \cdot \sum_{m=1,m \neq i}^{M}e_{k m}, & if \ k =j
\end{array}\right.
\end{equation}
In Eqn.4, when calculating negative similarity ($k \neq j$), the centroid $d_{k}$ is the average of all the
semantic embeddings of $k$th audio, while when calculating positive similarity ($k = j$), we eliminate $e_{ki}$ to compute the centroid.

During the training, we want the semantic embeddings of each audio to be similar to its centroid, but far from the centroid of other audios in the semantic space. As shown in the similarity matrix in Fig. 2, we want the similarity values of colored areas to be large, and the values of blank areas to be small. So for each semantic embedding, the loss function is designed as:
\begin{equation}
L\left(\mathbf{e}_{j i}\right)=-{S}_{j i, j}+\log \sum_{k=1}^{N} \exp \left({S}_{j i, k}\right).
\end{equation}

After the training of stage 1 is completed, we extract the centroid of each audio to represent its caption semantic embedding.
\subsubsection{Training details}
In this stage, we use a single-layer, bi-directional LSTM network followed by a linear fully connected layer, The dimensions of the LSTM and linear layer are 1024 and 512, respectively. When training the  model, each batch contains $N$ = 64 audios and $M$ = 3 caption per audios. We train the network with Adam optimizer using a learning rate of 0.01, and the total number of training epochs is 500. The scaling factors ($w$,$b$) are initialized as ($10$,$-5$).
\vspace{-20pt}
\subsection{Stage 2:Regularize the generation of captions}

As shown in Fig. 1, the caption semantic embedding $d_k$ is used in the semantic constraint module to regularize the generation of the caption.

We obtain the semantic embedding of the predicted caption by averaging pooling and max pooling operations on the decoder output representation $H$ along the time axis, as shown in the following equation:
\begin{equation}
    \hat{e}_{k}(\theta,x) = Mean\left (H(\theta,x) \right ) + Max\left ( H(\theta,x) \right ),
\end{equation}
where $\hat{e}_{k}$ is the semantic embedding of the $k$th audio predicted caption.

In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity (see Equation 7). 
\begin{equation}
    \ell_{SC}(\omega  ; d_{k}, x) = 1 - cosine\_similarity(\hat{e}_{k},d_{k}),
\end{equation}
 In this way, a small loss means $\hat{e}_{k}$ has high similarity with the audio caption semantic embedding $d_{k}$ obtained by stage 1.

Accordingly, the final training objective function is the weighted sum of cross-entropy loss and semantic constraint loss, where $\lambda$ is a hyperparameter.
\begin{equation}
 \ell(\omega; d_{k}, c, x) = \ell_{\mathrm{CE}}(\theta  ; c, x) + \lambda \cdot \ell_{SC}(\theta  ; d_{k}, x)
\end{equation}

\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}%
\setlength\tabcolsep{3pt}
    \centering
    \caption{Experimental results  under Clotho-v1 and Clotho-v2 evaluation sets}

    \begin{tabular}{c|c|cc|ccccccc}\toprule 
         Dataset&Model&Encoder&Decoder&BLEU$_1$&BLEU$_4$&ROUGE$_L$&METER&CIDEr&SPICE&SPIDEr \\\midrule 
         \multirow{11}{*}{\rotatebox{90}{Clotho-v1}}&\multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&53.7&14.1&35.9&16.4&33.5&11.1&22.3 \\
         & & & Transformer&53.4&13.2&35.5&{16.0}&31.7&11.0&21.3\\\cline{3-4}
         & &\multirow{2}{*}{Pretrain-CNN}&GRU&54.3&14.6&36.3&16.8&36.6&\textcolor{blue}{11.7}&{24.1}\\
         && &Transformer&54.8&15.0&36.4&16.7&33.4&11.0&22.2\\\cline{2-11}
         & AT-CNN~\cite{xu2021investigating}&Pretrain-CNN&GRU&\textcolor{blue}{55.6}&\textcolor{red}{15.9}&{36.8}&{16.9}&\textcolor{red}{37.7}&{11.5}&\textcolor{blue}{24.6}\\
         & Fine-tune PreCNN Transformer~\cite{chen2020audio}&CNN&Transformer&53.4&15.1&35.6&16.0&34.6&10.8&22.7\\
         & Temporal attention model~\cite{helinautomated}&CNN&LSTM&48.9&10.7&32.5&14.8&25.2&9.1&17.2\\\cline{2-11} 
         & \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.5}&{15.2}&{36.7}&\textcolor{red}{17.0}&{36.7}&{11.5}&{24.1}\\
         & & & Transformer&\textcolor{red}{55.8}&\textcolor{red}{15.9}&\textcolor{red}{37.3}&16.8&35.8&11.5&23.6\\  \cline{3-4}
         & &\multirow{2}{*}{Pretrain-CNN}&GRU&\textcolor{red}{55.8}&\textcolor{blue}{15.7}&\textcolor{blue}{36.9}&\textcolor{red}{17.1}&\textcolor{blue}{37.6}&\textcolor{red}{11.8}&\textcolor{red}{24.7}\\
         & & & Transformer&55.0&15.3&36.8&16.8&34.3&11.2&22.7\\ \hline \hline
         
        \multirow{11}{*}{\rotatebox{90}{Clotho-v2}}&\multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&54.9&15.0&{37.2}&17.1&37.4&11.8&24.5 \\
        & & & Transformer&54.8&15.3&37.8&{16.8}&35.8&11.3&23.6\\\cline{3-4}
        & &\multirow{2}{*}{Pretrain-CNN}&GRU&55.4&15.1&36.8&{17.4}&39.0&11.9&25.5\\
        & & &Transformer&55.8&15.9&37.3&16.8&35.8&11.5&23.6\\\cline{2-11}
        & AT-CNN~\cite{xu2021sjtu}&Pretrain-CNN&GRU&\textcolor{red}{56.5}&{15.5}&{37.4}&{17.4}&{39.9}&11.9&{25.9}\\
        & Transformer+RNN-LM~\cite{narisetty2021leveraging}&PANN&Transformer+RNN-LM&53.3&14.6&35.5&15.4&34.1&10.6&22.4\\
        & CL4AC~\cite{liu2021cl4ac}&PANN&Transformer&55.3&14.3&{37.4}&16.8&36.8&11.5&24.2\\\cline{2-11}
        & \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.8}&{16.1}&\textcolor{blue}{37.6}&\textcolor{red}{17.6}&{39.5}&{12.1}&{25.8}\\
        & & & Transformer&56.3&15.0&37.1&\textcolor{blue}{17.6}&37.0&11.9&24.4\\  \cline{3-4}
        & &\multirow{2}{*}{Pretrain-CNN}&GRU&\textcolor{blue}{56.4}&\textcolor{blue}{16.5}&\textcolor{red}{37.7}&\textcolor{red}{17.7}&{41.3}&{12.1}&{26.7}\\
        & & & Transformer&56.3&\textcolor{red}{16.7}&\textcolor{blue}{37.6}&17.0&37.6&11.4&24.5\\\bottomrule
    \end{tabular}
    \vspace{-13pt}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Experimental results  under Clotho-v2 evaluation set}

%     \begin{tabular}{c|cc|ccccccc}\toprule 
%          Model&Encoder&Decoder&BLEU$_1$&BLEU$_4$&ROUGE$_L$&METER&CIDEr&SPICE&SPIDEr \\\midrule 
%          \multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&54.9&15.0&{37.2}&17.1&37.4&11.8&24.5 \\
%          & & Transformer&54.8&15.3&37.8&{16.8}&35.8&11.3&23.6\\\cline{2-3}
%          &\multirow{2}{*}{Pretrain-CNN}&GRU&55.4&15.1&36.8&{17.4}&39.0&11.9&25.5\\
%          & &Transformer&55.8&15.9&37.3&16.8&35.8&11.5&23.6\\\midrule 
%          AT-CNN~\cite{xu2021sjtu}&Pretrain-CNN&GRU&{56.5}&{15.5}&{37.4}&{17.4}&{39.9}&11.9&{25.9}\\
%          Transformer+RNN-LM~\cite{narisetty2021leveraging}&PANN&Transformer+RNN-LM&53.3&14.6&35.5&15.4&34.1&10.6&22.4\\
%          CL4AC~\cite{liu2021cl4ac}&PANN&Transformer&55.3&14.3&{37.4}&16.8&36.8&11.5&24.2\\\midrule 
%          \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.8}&{16.1}&{37.6}&{17.6}&{39.5}&{12.1}&{25.8}\\
%          & & Transformer&56.6&15.0&37.1&17.6&37.0&11.9&24.4\\  \cline{2-3}\cline{2-3}
%           &\multirow{2}{*}{Pretrain-CNN}&GRU&{56.4}&{16.5}&{37.7}&{17.7}&{41.3}&{12.1}&{26.7}\\
%           & & Transformer&57.3&16.7&37.6&17.0&37.6&11.4&24.5\\ \bottomrule
%     \end{tabular}
% \end{table*}


In this stage, we apply SpecAugment~\cite{park2019specaugment} before feeding the audio feature to the model. Label smoothing~\cite{szegedy2016rethinking} is applied to smooth the one-hot word label. We also apply scheduled sampling to gently decrease the training-inference discrepancy caused by teacher forcing training~\cite{bengio2015scheduled}. The output dimensions of the decoder are 512 and the Transformer decoder has 4 heads. As for the GRU decoder, we train the network with Adam optimizer using the initial learning rate $5\times10^{-4}$, and the total number of training epochs is 25. And for the Transformer decoder, the initial learning rate is $5\times10^{-3}$ and warm-up is used in the first 5 epochs to increase the learning rate to the initial learning rate linearly. The total number of training epochs is 30 and the learning rate is then decreased to 1/10 of itself every 10 epochs. $\lambda$ is $0.5$.


==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Related_Work.tex <==
\vspace{-15pt}
\section{Related Work}
The audio captioning task is first introduced in~\cite{drossos2017automated}, which proposed the commercial ProSound Effects~\cite{lipping2019crowdsourcing} audio corpus as a proof of concept. The paper proposed a BiGRU~\cite{rana2016gated} based encoder-decoder model to generate audio captions. And due to the success of the audio captioning task in DCASE 2020 and 2021~\cite{Drossos_2019_dcase}, this task has garnered the attention of an increasing number of researchers, several papers and methods to address this issue have been proposed. H. Wang et al.~\cite{helinautomated} proposed a temporal attention mechanism in the decoder, which could utilize more acoustic information for each time step. K. Chen et al.~\cite{chen2020audio} used the combination of a pre-trained encoder and a Transformer decoder which makes the latent variable resulted more efficient in generating captions. X. Xu et al.~\cite{xu2021investigating} investigated the impact of local and global information on the audio captioning task by comparing two pre-training tasks. The semantic information is also studied to improve the performance of the audio captioning task. the semantic attributes are firstly used in ~\cite{kim2019audiocaps}, which used AudioSet labels as semantic attributes by using the labels of the nearest video clip. And  Eren et al. ~\cite{eren2020audio} used the audio encoder to get audio embeddings and text encoder to get subject-verb embeddings, combine these embeddings and decode them in the decoder.


==> Caption Feature Space Regularization for Audio Captioning (SPL) -arxiv/Contents/Title.tex <==
\title{Audio Captioning with Two-Stage Caption Semantic Consistency Constraint}
 %\IEEEmembership{Fellow, IEEE}
\author{Yiming Zhang, Hong Yu, Ruoyi Du, Zhanyu Ma, \IEEEmembership{Senior Member, IEEE}, Yuan Dong
\thanks{This work was supported in part by the National Key R\&D Program of China under Grant 2019YFF0303300 and under Subject II No. 2019YFF0303302, in part by National Natural Science Foundation of China (NSFC) under Grant 61922015, U19B2036, in part by Beijing Natural Science Foundation Project under Grant Z200002.}
\thanks{Y. Zhang, R. Du, Z. Ma, D.Yuan are with the Pattern Recognition and Intelligent System Laboratory, School of Artificial Intelligence, Beijing University of Posts and Telecommunications, Beijing 100876,
China. E-mail: \{zhangyiming, beiyoudry, mazhanyu, yuandong\}@bupt.edu.cn}
\thanks{S. B. Author, Jr., was with Rice University, Houston, TX 77005 USA. He is now with the Department of Physics, Colorado State University, Fort Collins, CO 80523 USA (e-mail: author@lamar.colostate.edu).}}
\markboth{Journal of \LaTeX\ Class Files, Vol. XX, No. X, August }
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
 \maketitle

==> Contents/Abstract.tex <==
\begin{abstract}
% The goal of the audio captioning task is to create a description of the audio clips' contents. Due to the ambiguity of audio, multiple people may perceive the same audio differently, resulting in caption disparities. However, because the audio captioning task uses a one-to-many training strategy, the disparity in captions has an impact on description generation, causing the network to become unstable. So in order to solve this problem, we propose a two-stage caption semantic consistency constraint method for audio captioning. Stage 1 use contrast learning to construct the caption semantic space and extract the caption semantic embedding, while stage 2 employs the  semantic embedding to regularize caption generation and reduce the effects of training approach and disparity. We conducted extensive experiments on two datasets using four commonly used encoder and decoder models. Experimental results indicate that the effectiveness of our proposed method in the metrics.

Audio captioning aims at describing the content of audio clips with human language. Due to the ambiguity of audio, multiple people may perceive the same audio differently, resulting in caption disparities (\emph{i.e.}, one audio may correlate to several captions with diverse semantics). For that, general audio captioning models achieve the one-to-many training by randomly selecting a correlated caption as the ground truth for each audio. However, it leads to a significant variation in the optimization directions and weakens model stability. To eliminate this negative impact, in this paper,  we propose a two-stage framework for audio captioning: (i) in the first stage, via a caption consistency regularization, we construct a proxy feature space to reduce distances between captions correlate to the same audio, and (ii) in the second stage, the proxy feature space is used as additional supervision to encourage the model to be optimized in a direction that benefits all correlated captions. We conducted extensive experiments on two datasets using four commonly used encoder and decoder architectures. Experimental results indicate the effectiveness of our proposed method in the metrics.
\end{abstract}

\begin{IEEEkeywords}
Audio captioning, contrastive learning, cross-modal task, semantic consistency constraint
\end{IEEEkeywords}


==> Contents/Conclusion.tex <==
\vspace{-10pt}
\section{Conclusion}
In this paper, we propose a two-stage caption semantic consistency constraint method for the audio captioning task, in which stage 1 uses contrast learning to extract the common semantic embedding of audio captions and stage 2 uses the extracted semantic embedding to regular the generated of caption and mitigate the impact of the caption disparity. We perform experiments using four different combinations of pre-trained encoders and decoders on two datasets to demonstrate the performance and effectiveness of our approach. According to the results, our best model performs competitive performance to the SOTA method on the Clotho-v1 dataset and outperforms the SOTA method on the Clotho-v2 dataset.

==> Contents/Experiments.tex <==
\vspace{-15pt}
\section{Experiments}
\vspace{-10pt}
\subsection{Metrics}
We evaluate the performance of our proposed method using the same metrics adopted in the DCASE Challenge, including machine translation metrics: BLEU$_n$~\cite{papineni2002bleu}, METEOR~\cite{banerjee2005meteor}, ROUGE$_L$~\cite{lin2004rouge} and captioning metrics: CIDEr~\cite{vedantam2015cider}, SPICE~\cite{anderson2016spice}, SPIDEr~\cite{liu2017improved}. 

The machine translation metrics are used to measure the word accuracy and recall of generated text compared to the ground truth, $n$ in BLEU means $n-$gram. And the captioning metrics are designed for the captioning task, which takes into account the scene graph inside the generated caption and the term frequency-inverse document frequency (TF-IDF) of the n-gram. By considering the scene graph and the TF-IDF of n-gram, ensuring semantic fidelity and syntactic fluency of the generated captions.
\vspace{-10pt}
\subsection{Datasets}

The Clotho dataset~\cite{drossos2020clotho} and the Audiocaps dataset~\cite{kim2019audiocaps} are two datasets that are commonly used for audio captioning tasks. There are two versions of the Clotho dataset, Clotho-v1 and Clotho-v2 respectively. each audio clip has five captions describing the audio contents, and the annotator uses only the audio signal for annotation. However, the Audiocaps dataset is not generated in an ideal environment, where annotators are provided with word labels and video information in addition to the audio signal~\cite{kim2019audiocaps}. So in this work,we only focus on the Clotho-v1 and Clotho-v2 datasets.
\vspace{-10pt}
\subsection{Experimental results}
Table I illustrates the experimental results of the proposed method compared to the baseline model and other methods on the Clotho-v1 and Clotho-v2 evaluation sets.

In each table, the first major column shows the experimental results of baseline models with different combinations of encoders and decoders, and the second major column is the result of other state of the art methods, where the baseline model using Pretrain-CNN encoder and attention-based GRU decoder is our implementation of the AT-CNN method. And the last major column is the experimental results of our proposed semantic consistency constraint method.

\subsubsection{Compared with baseline models}In both two datasets, our proposed semantic consistency constraint methods outperform the baseline models in the same encoder and decoder models. When compared to the SOTA model, AT-CNN, our best model which the encoder is Pretrain-CNN and the decoder is GRU, performs similarly on the Clotho-v1 dataset and outperforms it on the Clotho-v2 dataset.

\subsubsection{Compared with other methods}From the results, our proposed model has a generally higher performance improvement on the Clotho-v2 dataset compared to Clotho-v1 in terms of captioning metrics. We believe this is because the Clotho-v2 dataset is larger than the Clotho-v1 dataset, which aids in the extraction of caption semantic embedding in stage 1 and hence minimizes the impact of caption disparity on caption creation and enabling the generated captions to achieve better performance in captioning metrics.




==> Contents/Introduction.tex <==
\vspace{-15pt}
\section{Introduction}

\IEEEPARstart{a}{udio}  captioning is an inter-modal translation task that requires extracting features from audio and combining them with a language model to describe the contents of audio~\cite{drossos2017automated,drossos2020clotho,koizumi2020transformer}. However, unlike the speech recognition task that transcribes speech to text~\cite{xu2021audio}, the audio captioning task focuses on recognizing human-perceived information in general audio signals and expressing it in text using natural language. The information includes the sound event, the acoustic scene, and high-level semantic information such as concepts, physical properties, and high-level knowledge~\cite{drossos2020clotho}.

% The audio captioning task is first introduced in~\cite{drossos2017automated}, which proposed the commercial ProSound Effects~\cite{lipping2019crowdsourcing} audio corpus as a proof of concept. The paper proposed a BiGRU~\cite{rana2016gated} based encoder-decoder model to generate audio captions. And due to the success of the audio captioning task in DCASE 2020 and 2021~\cite{Drossos_2019_dcase}, this task has garnered the attention of an increasing number of researchers, several papers and methods to address this issue have been proposed. H. Wang et al.~\cite{helinautomated} proposed a temporal attention mechanism in the decoder, which could utilize more acoustic information for each time step. K. Chen et al.~\cite{chen2020audio} used the combination of a pre-trained encoder and a Transformer decoder which makes the latent variable resulted more efficient in generating captions. X. Xu et al.~\cite{xu2021investigating} investigated the impact of local and global information on the audio captioning task by comparing two pre-training tasks. The semantic information is also studied to improve the performance of the audio captioning task. the semantic attributes are firstly used in ~\cite{kim2019audiocaps}, which used AudioSet labels as semantic attributes by using the labels of the nearest video clip. And  Eren et al. ~\cite{eren2020audio} used the audio encoder to get audio embeddings and text encoder to get subject-verb embeddings, combine these embeddings and decode them in the decoder.

Different from the visual captioning tasks in which people can easily describe the visual object by its shape, color, size, and its position relative to other objects~\cite{wu2019audio}. However, for the audio sounds, its information can be much more ambiguous than the information in the image or video~\cite{drossos2020clotho,wu2019audio}. Even people find it challenging to precisely detect the events in an audio signal. Furthermore, it is difficult to determine the ideal description for the given audio because the description is often dependent on the situation or context as much as the sound itself. But due to the ambiguity of audio, different persons may have varying perceptions of the same sounds, resulting in the semantic disparity of audio captions~\cite{drossos2020clotho}, for example, a thin plastic rattling could be perceived as a fire crackling~\cite{lipping2019crowdsourcing}.

In the audio captioning task, each audio has multiple captions to describe the contents, and one caption for each training is randomly selected as the objective for the model to generate a description of the audio clip. However, due to the disparity of captions, randomly selecting one caption as the objective during each training will lead to a large variance in the optimization direction of the model, which may have a significant impact on the performance of the model and make it more difficult to train.
% \textcolor{blue}{However due to the disparity of captions, this one-to-many training strategy may have a significant impact on the performance of the model and make it more difficult to train. }

To solve the problem caused by the disparity of captions, the most intuitive way is to feed all captions of each audio simultaneously as optimization objectives into the network at the same time for training, but this approach leads to a multiply increasing memory, which is not an acceptable solution with limited computational resources.

\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_2.png}}
\caption{The system overview of our proposed method. The mainstream encoder-decoder audio captioning framework is in the yellow block, and in the green block is our proposed  caption semantic consistency constraint module which is described in sections B and C.}
\vspace{-13pt}
\end{figure*}
So we choose not to impose this stability constraint at the model output level, but to reconstruct such a constraint in the feature space. We propose a two-stage caption semantic consistency constraint method. Our proposed method includes two-stage: stage 1 generates the semantic space of the captions by minimizing the distance between different captions belonging to the same audio and pushing away the distance between different captions of different audio. And stage 2 regularizes the creation of audio descriptions by using the semantic feature space generated in stage 1 as our optimization objective.

% the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and extract the common caption semantic embedding of each audio. And in order to mitigate the influence of the training strategy, stage 2 regularizes the generation of audio captions using the extracted caption semantic embedding.


Our contributions are as follows:
\begin{itemize}
  \item [1)] We propose a two-stage caption semantic consistency constraint approach to mitigate the impact of caption disparity on audio captioning tasks.
  \item [2)]Two different pre-trained encoders and two different decoders are used to verify the effectiveness of the method.
  \item [3)]On two prominent audio captioning datasets, Clotho-v1 and Clotho-v2~\cite{drossos2020clotho}, the results of our proposed method are compared to the results of the state of the arts, indicating that our proposed method achieves competitive results.
\end{itemize}

% The remainder of this paper is organized as follows. We introduce our proposed method in Section 2. Experiments are described in Section 3. Results are shown in Section 4. Finally, we conclude our work in Section 5.


==> Contents/Method.tex <==
% \begin{figure*}
% \centerline{\includegraphics[width=14cm]{stage_1.pdf}}
% \caption{The system overview of stage 1. Different colors indicate caption embeddings from different audios.}
% \end{figure*}
\section{Proposed Method}
The proposed model, which is a two-stage method, is described in this section. Stage 1 uses contrast learning to extract the common semantic embedding of audio captions, reducing the impact of caption semantic disparity. Stage 2 constrains the generated audio description using the extracted semantic embedding.
\subsection{Stage 1:The extraction of caption semantic embedding}
To reduce the impact of caption disparity on model training due to training strategy. We use the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and increase the semantic space distance between captions that belong to different audio.
\subsubsection{Training method}
As is depicted in Fig. 1, $N \times M$ captions are fetched to build a batch. These captions are from $N$ different audios, and each audio has $M$ captions. The symbol $t_{ji}$ ($1 \le j \le N$ and $1 \le i \le M$) represents the $i$th caption from the $j$th audio. 

We tokenize the captions and utilize Bert~\cite{devlin2018bert} to extract the its word embeddings. And then the word embeddings are fed into an LSTM network. A linear layer is connected to the LSTM layer as an additional transformation of the network. We denote the output of the entire neural network as $ G\left ( t_{ji};w \right ) $ where $w$ represents all parameters of the neural network. The caption embedding vector is defined as:
\begin{equation}
e_{ji} = Mean\left ( G\left ( t_{ji};w \right ) \right ) + Max\left ( G\left ( t_{ji};w \right ) \right ),
\end{equation}
here $e_{ji}$ represents semantic embedding of the $j$th audio’s $i$th caption. 

The centroid of the semantic embeddings from the $j$th audio $\left [ e_{j1},\cdots ,e_{jM} \right ] $ is denoted as $c_{j}$, and the similarity matrix $S_{ji,k}$ is defined as the scaled cosine similarities between each semantic embedding $e_{ji}$ to all centroids $c_{k}$ ($1 \le j, k \le N$ and $1 \le i \le M$):
\begin{equation}
S_{ji,k}= w \cdot cosine\left ( e_{ji},c_{k} \right ) +b ,
\end{equation}
where $w$ and $b$ are learnable parameters, the weight are constrained to be positive ($w > 0$). And the centroid $c_{k}$ can be calculated by:
\begin{equation}
c_{k} = \left\{\begin{array}{ll}
\frac{1}{M} \cdot \sum_{m=1}^{M}e_{k m},&if \ k \neq j  \\
\frac{1}{M-1} \cdot \sum_{m=1,m \neq i}^{M}e_{k m}, & if \ k =j
\end{array}\right.
\end{equation}
In Eqn.3, when calculating negative similarity ($k \neq j$), the centroid $c_{k}$ is the average of all the
semantic embeddings of $k$th audio, while when calculating positive similarity ($k = j$), we eliminate $e_{ki}$ to compute the centroid.

During the training, we want the semantic embeddings of each audio to be similar to its centroid, but far from the centroid of other audios in the semantic space. As shown in the similarity matrix in Fig. 1, we want the similarity values of colored areas to be large, and the values of blank areas to be small. So for each semantic embedding, the loss function is designed as:
\begin{equation}
L\left(\mathbf{e}_{j i}\right)=-\mathbf{S}_{j i, j}+\log \sum_{k=1}^{N} \exp \left(\mathbf{S}_{j i, k}\right).
\end{equation}

After the training of stage 1 is completed, we extract the centroid of each audio to represent its caption semantic embedding.
\subsubsection{Training details}
In this stage, we use a single-layer, bi-directional LSTM network followed by a linear fully connected layer, The dimensions of the LSTM and linear layer are 1024 and 512, respectively. When training the  model, each batch contains $N$ = 64 audios and $M$ = 3 caption per audios. We train the network with Adam optimizer using a learning rate of 0.01, and the total number of training epochs is 500. The scaling factors ($w$,$b$) are initialized as ($10$,$-5$).
\subsection{Stage 2:The generation of audio captioning}
%总述目前的模型一般Seq2Seq的
Existing audio captioning systems are usually based on an encoder-decoder framework, as shown in Fig. 2. In the encoder, the audio data is encysted into a latent representation, and then the representation is fed to the decoder for word-level prediction to generate captions for audio.
\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_2.pdf}}
\caption{The system overview of stage 2. }
\end{figure*}

Typically, the encoder employs pre-trained models that have been trained in advance for sound event detection or sound scene recognition tasks, such as PANN~\cite{kong2020panns}, VGGish~\cite{hershey2017cnn}, or Pretrain-CNN~\cite{xu2021investigating}. And the decoder is an autoregressive language model, like Transformer or GRU, which is trained from scratch.
\subsubsection{Encoder}
In our work, we used two different 10-layer CNN pre-training models, PANN and Pretrain-CNN, and the model structures are shown in Table I.
% \begin{table}[h]
%     \caption{Caption}
%     \label{tab:my_label}
%     \centering
%     \begin{tabular}{c|c}\hline
%     PANN & Pretrain-CNN\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                         3 \times 3 @ 64 \\ BN, ReLU 
%                         \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                     3 \times 3 @ 128 \\ BN, ReLU 
%                     \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%                 3 \times 3 @ 256 \\ BN, ReLU 
%                 \end{array}\right) \times 2$}\\\hline
%     \multicolumn{2}{c}{Pooling$\  2\times 2$}\\ \hline
%     \multicolumn{2}{c}{$\left(\begin{array}{c}
%             3 \times 3 @ 512 \\ BN, ReLU 
%             \end{array}\right) \times 2$}\\\hline
%     Global pooling & Pooling with length  \\\hline
%     \multicolumn{2}{c}{FC 512,ReLU}\\\hline
%     \multicolumn{2}{c}{FC 527, Sigmoid}\\\hline
    
%     \end{tabular}

% \end{table}

Both PANN~\cite{kong2020panns} and Pretrain-CNN~\cite{xu2021investigating} are pre-trained on Audioset, the world's biggest sound event detection dataset. The distinction is that Pretrain-CNN computes the representation using the actual length of each audio feature, whereas PANN during training uses the longest length in the batch.

\subsubsection{Decoder}We use a single-layer attention-based  GRU~\cite{bahdanau2014neural} and 2 layers transformer~\cite{vaswani2017attention} as our backbone decoder for its success in previous audio captioning works.

% \emph{GRU Decoder:} At the each decoding step $n$, the hidden state $h_{n}$ is updated depending on the previous timestep $h_{n-1}$, and the concatenation of the current input word token $t_{n}$ and a context vector $v_{n}$:
% \begin{equation}
% h_{n}=GRU\left(\left[v_{n} ;WE\left(t_{n}\right)\right], h_{n-1}\right),
% \end{equation}
% where $WE$ denotes the word embedding layer. A standard temporal attention mechanism is utilized to obtain $v_n$ the attention weights $\left \{\alpha_{n,t} \right \} ^{T}_{t=1}$ can be calculated by $h_{n-1}$ and the audio representation:
% \begin{equation}
%     \alpha_{n, t}=\frac{\exp \left(score\left(\mathbf{h}_{n-1}, \mathbf{e}_{t}\right)\right)}{\sum_{t=1}^{T^{\star}} \exp \left(score\left(\mathbf{h}_{n-1}, \mathbf{e}_{t}\right)\right)},
% \end{equation}
% \begin{equation}
%     v_{n}= {\sum_{t=1}^{T}\alpha_{n, t}\cdot e_{t}}.
% \end{equation}

% \emph{Transformer Decoder:} In our work, we use the typical 2 layers  Transformer decoder, The detailed
% structure of Transformer can be found \textcolor{blue}{in}.

% \textcolor{blue}{The word embedding of the token is fed into the decoder. The input is delivered to the masked multi-head attention module, which generates a query vector feature using a decoder layer. The value vector is then used as an input to the subsequent multi-head attention module. Additionally, the multi-head attention module uses encoder output as the key vector and value vector inputs. We may retrieve the output of a decoder layer after layer norm and feedforward module. Each decoder layer employs a skip connection method to avoid gradient vanishing difficulties. Finally, the decoder's output is transferred to a linear layer and a softmax function to obtain the caption words' output probabilities.}
\subsubsection{Loss}
We use the combination of two loss functions in the training, the standard cross-entropy loss  and the semantic constraint loss.

\emph{Cross-entropy Loss:} The cross-entropy loss function is used for word-level classification, for the same reason as other audio captioning methods use. Given the acoustic feature $F$ of the audio, the parameters of the model are $w$, the loss function is:
\begin{equation}
    \ell_{\mathrm{CE}}(\omega  ; S, F)=-\sum_{t=1}^{T} \log p\left(S_{t} \mid \omega , F\right),
\end{equation}
where $S$ is the objective caption of the audio and $S_{t}$ is the expected word at time $t$.

\emph{Semantic Constraint Loss:} We obtain the semantic embedding of the generated caption by averaging pooling and max pooling operations on the decoder output feature $H$ along the time axis, as shown in the following equation:
% In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity. 
% We obtain the semantic embedding of the generated caption by averaging pooling and max pooling operations on the decoder output feature $H$ along the time axis, as shown in the following equation:
\begin{equation}
    \hat{e}_{k}(\omega,F) = Mean\left (H(\omega,F) \right ) + Max\left ( H(\omega,F) \right ),
\end{equation}
where $\hat{e}_{k}$ is the semantic embedding of the $k$th audio generated caption.

In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity (see Equation 10). 
\begin{equation}
    \ell_{SC}(\omega  ; c_{k}, F) = 1 - cosine\_similarity(\hat{e}_{k},c_{k}),
\end{equation}
 In this way, a small loss means $\hat{e}_{k}$ has high similarity with the audio caption semantic embedding $c_{k}$ obtained by stage 1.
 
Accordingly, the final training objective function is the weighted sum of cross-entropy loss and semantic constraint loss, where $\lambda$ is a hyperparameter.
\begin{equation}
 \ell(\omega; c_{k}, S, F) = \ell_{\mathrm{CE}}(\omega  ; S, F) + \lambda \cdot \ell_{SC}(\omega  ; c_{k}, F)
\end{equation}

\subsubsection{Training details} \textcolor{blue}{In this stage, we apply SpecAugment~\cite{park2019specaugment} before feeding the audio feature to the model. Label smoothing~\cite{szegedy2016rethinking} is applied to smooth the one-hot word label. We also apply scheduled sampling to gently decrease the training-inference discrepancy caused by teacher forcing training~\cite{bengio2015scheduled}. The probability of feeding the ground truth word to the decoder is linearly decayed from 1.0 to 0.7. We train the network with Adam optimizer using initial learning rate $5e^{-5}$, and the total number of training epochs is 25. }


==> Contents/NewMethod.tex <==
\vspace{-15pt}
\section{Proposed Method}

\subsection{The overview of audio captioning system}
the current mainstream training paradigm of the audio captioning task is the end-to-end encoder-decoder framework, as shown in the yellow block of Fig. 1.

The training data for the task consists of paired audio and captions data. We denote a training set of $N$ audio-captions pair $D=\left\{\left(x_{n}, C_{n}\right)\right\}_{n=1}^{N}$, where $x\in {R}^{T \times F}$ is the log mel-spectrogram of the audio clip with $T$ frames and $F$ Mel filters, $C_n=\left\{c_{mn}^{L}\right\}_{m=1}^{M}$ is all the captions of the $n$th audio clip, and $c_{mn}^{L}$ is the $m$-th caption having $L$ tokens.

The audio encoder takes the log mel-spectrogram $x$ of an audio clip as the input and extracts its latent representation $z\in {R}^{T^{\prime} \times F^{\prime}}$. Then latent representation $z$ is aligned and calculated with the hidden states of tokens by the decoder, the caption representation can be calculated by the decoder, denoted as $H \in {R}^{L \times D}$, which contains $L$ vectors $\left\{h_l\right\}_{l=1}^{L}$, where the dimension of $h_l$ is $D$ and the  number of vectors is equal to the token length of caption $c$. Hence, each vector $h_l$ corresponds to the token $c^l$ in the objective caption, and then the vectors are  used to predict the probability of the words over the vocabulary after it is passed through the  linear layer with softmax function.The predicted words are $\left\{w_l\right\}_{l=1}^{L}$.

The cross-entropy loss function is used for word-level classification of decoder, the loss function is:
\begin{equation}
    \ell_{\mathrm{CE}}(\theta  ; c, x)=-\sum_{l=1}^{L} c^l \cdot \log p\left(w_{l} \mid \theta, x\right),
\end{equation}


\subsubsection{Encoder}
The encoder employs pre-trained models that have been trained in advance for sound event detection or sound scene recognition tasks, such as PANN~\cite{kong2020panns}, VGGish~\cite{hershey2017cnn}, or Pretrain-CNN~\cite{xu2021investigating}. And in our work, we used two different 10-layer CNN pre-trained models, PANN and Pretrain-CNN, and the model structures of them can be found in ~\cite{kong2020panns,xu2021investigating}.

\subsubsection{Decoder}The decoder is usually a language model, like Transformer or GRU, which is trained from scratch. And during training, teacher forcing is used to accelerate the training process. In our work, we use a single-layer attention-based  GRU~\cite{bahdanau2014neural} and 2 layers transformer~\cite{vaswani2017attention} as our backbone decoder for its success in previous audio captioning works.

For the audio captioning task, an audio clip has multiple captions to describe how different annotators feel about it. Different perceptions cause the disparity of the captions, however, for each audio, only one caption will be randomly selected as the groundtruth for each training to generate the description of the audio, and this training strategy can easily affect the performance of the model and make it unstable.

To solve the above problem, we propose a caption semantic consistency constraint method to regularize the generation of the caption, the key module are shown in the green block of Figure 1. Our method is a two-stage audio captioning method, in which stage 1 uses contrast learning to generate the semantic space and extract the caption semantic embedding of each audio $d_k$ (described in section B) and then the semantic embedding $d_k$ is used in the module to regularize the generation of caption in stage 2 (described in section C).
\begin{figure*}
\centerline{\includegraphics[width=14cm]{stage_1.png}}
\caption{The system overview of stage 1. Different colors indicate caption embeddings from different audios. The colored areas are the positive similarity and the blank areas are negative in the similarity matrix.}
\vspace{-13pt}
\end{figure*}\textbf{}


\vspace{-10pt}
\subsection{Stage 1:The extraction of caption semantic embedding}
To reduce the impact of caption disparity on model training. We use the contrast learning method to reduce the semantic space distance between captions that belong to the same audio and increase the semantic space distance between captions that belong to different audio.

\subsubsection{Training method}
As is depicted in Fig. 2, $N \times M$ captions are fetched to build a batch. These captions are from $N$ different audios, and each audio has $M$ captions. The symbol $c_{ji}$ ($1 \le j \le N$ and $1 \le i \le M$) represents the $i$th caption from the $j$th audio. 

We tokenize the captions and utilize Bert~\cite{devlin2018bert} to extract its word embeddings. And then the word embeddings are fed into an LSTM network. A linear layer is connected to the LSTM layer as an additional transformation of the network. We denote the output of the entire neural network as $ G\left ( c_{ji};w \right ) $ where $w$ represents all parameters of the neural network. The caption embedding vector is defined as:
\begin{equation}
e_{ji} = Mean\left ( G\left ( c_{ji};w \right ) \right ) + Max\left ( G\left ( c_{ji};w \right ) \right ),
\end{equation}
here $e_{ji}$ represents semantic embedding of the $j$th audio’s $i$th caption. 

The centroid of the semantic embeddings from the $j$th audio $\left [ e_{j1},\cdots ,e_{jM} \right ] $ is denoted as $d_{j}$, and the similarity matrix $S_{ji,k}$ is defined as the scaled cosine similarities between each semantic embedding $e_{ji}$ to all centroids $d_{k}$ ($1 \le j, k \le N$ and $1 \le i \le M$):
\begin{equation}
S_{ji,k}= w \cdot cosine\left ( e_{ji},d_{k} \right ) +b ,
\end{equation}
where $w$ and $b$ are learnable parameters, the weight are constrained to be positive ($w > 0$). And the centroid $c_{k}$ can be calculated by:
\begin{equation}
d_{k} = \left\{\begin{array}{ll}
\frac{1}{M} \cdot \sum_{m=1}^{M}e_{k m},&if \ k \neq j  \\
\frac{1}{M-1} \cdot \sum_{m=1,m \neq i}^{M}e_{k m}, & if \ k =j
\end{array}\right.
\end{equation}
In Eqn.4, when calculating negative similarity ($k \neq j$), the centroid $d_{k}$ is the average of all the
semantic embeddings of $k$th audio, while when calculating positive similarity ($k = j$), we eliminate $e_{ki}$ to compute the centroid.

During the training, we want the semantic embeddings of each audio to be similar to its centroid, but far from the centroid of other audios in the semantic space. As shown in the similarity matrix in Fig. 2, we want the similarity values of colored areas to be large, and the values of blank areas to be small. So for each semantic embedding, the loss function is designed as:
\begin{equation}
L\left(\mathbf{e}_{j i}\right)=-{S}_{j i, j}+\log \sum_{k=1}^{N} \exp \left({S}_{j i, k}\right).
\end{equation}

After the training of stage 1 is completed, we extract the centroid of each audio to represent its caption semantic embedding.
\subsubsection{Training details}
In this stage, we use a single-layer, bi-directional LSTM network followed by a linear fully connected layer, The dimensions of the LSTM and linear layer are 1024 and 512, respectively. When training the  model, each batch contains $N$ = 64 audios and $M$ = 3 caption per audios. We train the network with Adam optimizer using a learning rate of 0.01, and the total number of training epochs is 500. The scaling factors ($w$,$b$) are initialized as ($10$,$-5$).
\vspace{-20pt}
\subsection{Stage 2:Regularize the generation of captions}

As shown in Fig. 1, the caption semantic embedding $d_k$ is used in the semantic constraint module to regularize the generation of the caption.

We obtain the semantic embedding of the predicted caption by averaging pooling and max pooling operations on the decoder output representation $H$ along the time axis, as shown in the following equation:
\begin{equation}
    \hat{e}_{k}(\theta,x) = Mean\left (H(\theta,x) \right ) + Max\left ( H(\theta,x) \right ),
\end{equation}
where $\hat{e}_{k}$ is the semantic embedding of the $k$th audio predicted caption.

In addition to the cross-entropy loss, we proposed the semantic constraint loss to reduce the effect of the caption disparity (see Equation 7). 
\begin{equation}
    \ell_{SC}(\omega  ; d_{k}, x) = 1 - cosine\_similarity(\hat{e}_{k},d_{k}),
\end{equation}
 In this way, a small loss means $\hat{e}_{k}$ has high similarity with the audio caption semantic embedding $d_{k}$ obtained by stage 1.

Accordingly, the final training objective function is the weighted sum of cross-entropy loss and semantic constraint loss, where $\lambda$ is a hyperparameter.
\begin{equation}
 \ell(\omega; d_{k}, c, x) = \ell_{\mathrm{CE}}(\theta  ; c, x) + \lambda \cdot \ell_{SC}(\theta  ; d_{k}, x)
\end{equation}

\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}%
\setlength\tabcolsep{3pt}
    \centering
    \caption{Experimental results  under Clotho-v1 and Clotho-v2 evaluation sets}

    \begin{tabular}{c|c|cc|ccccccc}\toprule 
         Dataset&Model&Encoder&Decoder&BLEU$_1$&BLEU$_4$&ROUGE$_L$&METER&CIDEr&SPICE&SPIDEr \\\midrule 
         \multirow{11}{*}{\rotatebox{90}{Clotho-v1}}&\multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&53.7&14.1&35.9&16.4&33.5&11.1&22.3 \\
         & & & Transformer&53.4&13.2&35.5&{16.0}&31.7&11.0&21.3\\\cline{3-4}
         & &\multirow{2}{*}{Pretrain-CNN}&GRU&54.3&14.6&36.3&16.8&36.6&\textcolor{blue}{11.7}&{24.1}\\
         && &Transformer&54.8&15.0&36.4&16.7&33.4&11.0&22.2\\\cline{2-11}
         & AT-CNN~\cite{xu2021investigating}&Pretrain-CNN&GRU&\textcolor{blue}{55.6}&\textcolor{red}{15.9}&{36.8}&{16.9}&\textcolor{red}{37.7}&{11.5}&\textcolor{blue}{24.6}\\
         & Fine-tune PreCNN Transformer~\cite{chen2020audio}&CNN&Transformer&53.4&15.1&35.6&16.0&34.6&10.8&22.7\\
         & Temporal attention model~\cite{helinautomated}&CNN&LSTM&48.9&10.7&32.5&14.8&25.2&9.1&17.2\\\cline{2-11} 
         & \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.5}&{15.2}&{36.7}&\textcolor{red}{17.0}&{36.7}&{11.5}&{24.1}\\
         & & & Transformer&\textcolor{red}{55.8}&\textcolor{red}{15.9}&\textcolor{red}{37.3}&16.8&35.8&11.5&23.6\\  \cline{3-4}
         & &\multirow{2}{*}{Pretrain-CNN}&GRU&\textcolor{red}{55.8}&\textcolor{blue}{15.7}&\textcolor{blue}{36.9}&\textcolor{red}{17.1}&\textcolor{blue}{37.6}&\textcolor{red}{11.8}&\textcolor{red}{24.7}\\
         & & & Transformer&55.0&15.3&36.8&16.8&34.3&11.2&22.7\\ \hline \hline
         
        \multirow{11}{*}{\rotatebox{90}{Clotho-v2}}&\multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&54.9&15.0&{37.2}&17.1&37.4&11.8&24.5 \\
        & & & Transformer&54.8&15.3&37.8&{16.8}&35.8&11.3&23.6\\\cline{3-4}
        & &\multirow{2}{*}{Pretrain-CNN}&GRU&55.4&15.1&36.8&{17.4}&39.0&11.9&25.5\\
        & & &Transformer&55.8&15.9&37.3&16.8&35.8&11.5&23.6\\\cline{2-11}
        & AT-CNN~\cite{xu2021sjtu}&Pretrain-CNN&GRU&\textcolor{red}{56.5}&{15.5}&{37.4}&{17.4}&{39.9}&11.9&{25.9}\\
        & Transformer+RNN-LM~\cite{narisetty2021leveraging}&PANN&Transformer+RNN-LM&53.3&14.6&35.5&15.4&34.1&10.6&22.4\\
        & CL4AC~\cite{liu2021cl4ac}&PANN&Transformer&55.3&14.3&{37.4}&16.8&36.8&11.5&24.2\\\cline{2-11}
        & \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.8}&{16.1}&\textcolor{blue}{37.6}&\textcolor{red}{17.6}&{39.5}&{12.1}&{25.8}\\
        & & & Transformer&56.3&15.0&37.1&\textcolor{blue}{17.6}&37.0&11.9&24.4\\  \cline{3-4}
        & &\multirow{2}{*}{Pretrain-CNN}&GRU&\textcolor{blue}{56.4}&\textcolor{blue}{16.5}&\textcolor{red}{37.7}&\textcolor{red}{17.7}&{41.3}&{12.1}&{26.7}\\
        & & & Transformer&56.3&\textcolor{red}{16.7}&\textcolor{blue}{37.6}&17.0&37.6&11.4&24.5\\\bottomrule
    \end{tabular}
    \vspace{-13pt}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Experimental results  under Clotho-v2 evaluation set}

%     \begin{tabular}{c|cc|ccccccc}\toprule 
%          Model&Encoder&Decoder&BLEU$_1$&BLEU$_4$&ROUGE$_L$&METER&CIDEr&SPICE&SPIDEr \\\midrule 
%          \multirow{4}{*}{Baseline}&\multirow{2}{*}{PANN}&GRU&54.9&15.0&{37.2}&17.1&37.4&11.8&24.5 \\
%          & & Transformer&54.8&15.3&37.8&{16.8}&35.8&11.3&23.6\\\cline{2-3}
%          &\multirow{2}{*}{Pretrain-CNN}&GRU&55.4&15.1&36.8&{17.4}&39.0&11.9&25.5\\
%          & &Transformer&55.8&15.9&37.3&16.8&35.8&11.5&23.6\\\midrule 
%          AT-CNN~\cite{xu2021sjtu}&Pretrain-CNN&GRU&{56.5}&{15.5}&{37.4}&{17.4}&{39.9}&11.9&{25.9}\\
%          Transformer+RNN-LM~\cite{narisetty2021leveraging}&PANN&Transformer+RNN-LM&53.3&14.6&35.5&15.4&34.1&10.6&22.4\\
%          CL4AC~\cite{liu2021cl4ac}&PANN&Transformer&55.3&14.3&{37.4}&16.8&36.8&11.5&24.2\\\midrule 
%          \multirow{4}{*}{Ours}&\multirow{2}{*}{PANN}&GRU&{55.8}&{16.1}&{37.6}&{17.6}&{39.5}&{12.1}&{25.8}\\
%          & & Transformer&56.6&15.0&37.1&17.6&37.0&11.9&24.4\\  \cline{2-3}\cline{2-3}
%           &\multirow{2}{*}{Pretrain-CNN}&GRU&{56.4}&{16.5}&{37.7}&{17.7}&{41.3}&{12.1}&{26.7}\\
%           & & Transformer&57.3&16.7&37.6&17.0&37.6&11.4&24.5\\ \bottomrule
%     \end{tabular}
% \end{table*}


In this stage, we apply SpecAugment~\cite{park2019specaugment} before feeding the audio feature to the model. Label smoothing~\cite{szegedy2016rethinking} is applied to smooth the one-hot word label. We also apply scheduled sampling to gently decrease the training-inference discrepancy caused by teacher forcing training~\cite{bengio2015scheduled}. The output dimensions of the decoder are 512 and the Transformer decoder has 4 heads. As for the GRU decoder, we train the network with Adam optimizer using the initial learning rate $5\times10^{-4}$, and the total number of training epochs is 25. And for the Transformer decoder, the initial learning rate is $5\times10^{-3}$ and warm-up is used in the first 5 epochs to increase the learning rate to the initial learning rate linearly. The total number of training epochs is 30 and the learning rate is then decreased to 1/10 of itself every 10 epochs. $\lambda$ is $0.5$.


==> Contents/Related_Work.tex <==
\vspace{-15pt}
\section{Related Work}
The audio captioning task is first introduced in~\cite{drossos2017automated}, which proposed the commercial ProSound Effects~\cite{lipping2019crowdsourcing} audio corpus as a proof of concept. The paper proposed a BiGRU~\cite{rana2016gated} based encoder-decoder model to generate audio captions. And due to the success of the audio captioning task in DCASE 2020 and 2021~\cite{Drossos_2019_dcase}, this task has garnered the attention of an increasing number of researchers, several papers and methods to address this issue have been proposed. H. Wang et al.~\cite{helinautomated} proposed a temporal attention mechanism in the decoder, which could utilize more acoustic information for each time step. K. Chen et al.~\cite{chen2020audio} used the combination of a pre-trained encoder and a Transformer decoder which makes the latent variable resulted more efficient in generating captions. X. Xu et al.~\cite{xu2021investigating} investigated the impact of local and global information on the audio captioning task by comparing two pre-training tasks. The semantic information is also studied to improve the performance of the audio captioning task. the semantic attributes are firstly used in ~\cite{kim2019audiocaps}, which used AudioSet labels as semantic attributes by using the labels of the nearest video clip. And  Eren et al. ~\cite{eren2020audio} used the audio encoder to get audio embeddings and text encoder to get subject-verb embeddings, combine these embeddings and decode them in the decoder.


==> Contents/Title.tex <==
\title{Audio Captioning with Two-Stage Caption Semantic Consistency Constraint}
 %\IEEEmembership{Fellow, IEEE}
\author{Yiming Zhang, Hong Yu, Ruoyi Du, Zhanyu Ma, \IEEEmembership{Senior Member, IEEE}, Yuan Dong
\thanks{This work was supported in part by the National Key R\&D Program of China under Grant 2019YFF0303300 and under Subject II No. 2019YFF0303302, in part by National Natural Science Foundation of China (NSFC) under Grant 61922015, U19B2036, in part by Beijing Natural Science Foundation Project under Grant Z200002.}
\thanks{Y. Zhang, R. Du, Z. Ma, D.Yuan are with the Pattern Recognition and Intelligent System Laboratory, School of Artificial Intelligence, Beijing University of Posts and Telecommunications, Beijing 100876,
China. E-mail: \{zhangyiming, beiyoudry, mazhanyu, yuandong\}@bupt.edu.cn}
\thanks{S. B. Author, Jr., was with Rice University, Houston, TX 77005 USA. He is now with the Department of Physics, Colorado State University, Fort Collins, CO 80523 USA (e-mail: author@lamar.colostate.edu).}}
\markboth{Journal of \LaTeX\ Class Files, Vol. XX, No. X, August }
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
 \maketitle
